Natural Language Processing Methods to Identify Oncology Patients at High Risk for Acute Care with Clinical Notes

Clinical notes are an essential component of a health record. This paper evaluates how natural language processing (NLP) can be used to identify the risk of acute care use (ACU) in oncology patients, once chemotherapy starts. Risk prediction using structured health data (SHD) is now standard, but predictions using free-text formats are complex. This paper explores the use of free-text notes for the prediction of ACU instead of SHD. Deep Learning models were compared to manually engineered language features. Results show that SHD models minimally outperform NLP models; an l1-penalised logistic regression with SHD achieved a C-statistic of 0.748 (95%-CI: 0.735, 0.762), while the same model with language features achieved 0.730 (95%-CI: 0.717, 0.745) and a transformer-based model achieved 0.702 (95%-CI: 0.688, 0.717). This paper shows how language models can be used in clinical applications and underlines how risk bias is different for diverse patient groups, even using only free-text data.

==> parts/related_works.tex <==
\section{Related Work}
In this section we are going to present the related works. Initially, we will focus on machine learning models applied to oncology, afterwards we will discuss existing literature on uncertainty quantification, especially in medical AI on how it is currently used.

\subsection{Machine Learning for Acute Care Utilization}
Various previous works have focused on applying ML to EHRs to identify patients at risk of ACU. 
\citet{keiserboys1} introduced a model to predict hospitalization of patients based on two variables, albumin and sodium. Their proposed model achieved a ROC AUC score of their validation cohort was 0.69 (95\% CI, 0.62-0.75).
\citet{canadaboy} introduced the PROACCT score, which is a combination of cancer type and treatment regimen, age, and emergency department visits in the prior year. Their model achieves a ROC AUC of 0.67 (95\% CI, 0.66-0.69) on their own test cohort for 30 day ACU risk prediction. \citet{Daly2019AFF} developed a model that identifies patients at high risk for a potentially preventable acute
care visit, based on EHRs with 270 features, using a time-weighted LASSO logistic regression. They achieved a C-statistic of 0.65.\\
\citet{dylan_paper} analyzed a patient cohort on the risk of preventable ACU, after oncology patients start their chemotherapy. In their paper they select a study population which is subject to the OP-35 metric. Based on the patients dense EHRs, originally consisting of 760 variables (such as demographic factors, lab values, drug prescription, and procedure codes), they show that these can be used to predict the risk of impatient and ED visits, 30 days, 180 days, and 365 days after the patients start chemotherapy. In their studies they analyze multiple ML models, and  propose a LASSO logistic regression to be the most suitable solution for the problem, by achieving an ROC AUC score of 0.783 (95\%CI: 0.761-0.806) to predict ACU risk in the next 180 days. By using the $\ell_1$ penalty in their logistic regression model, they reduced the number of features to 125.\\

\subsection{Natural Language in Medicine}

